Keywords for Bias

This work proposes to analyse some keywords for bias analysis. For this, we are using several NLP approaches and compare them based on their capability of detecting keywords to analyse bias. The overall findings show that our proposed approach gives comparable results with the state-of-the-art approaches on different benchmark datasets.

==> discussion.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu


Before investigating the existence of bias in SERPs, we initially compared the retrieval performances of two search engines. In Table~\ref{tab:performance} we observe that the performance of the two search engines is high but engine 1 is better than engine 2 -- their difference is statistically significant. This is verified across all three IR evaluation measures. %This suggest that the search engines  %All three evaluation measures support that Engine 1 performs better in retrieving relevant documents, RBP with 99\% confidence (i.e., $\alpha = 0.01$) and other two measures even with higher confidence values.

%Symbols in the table were obtained from: http://www.apsstylemanual.org/apsHouseStyle/handEditing/tables.htm
%Finally, any statistical information indicated in the table by symbols should be described. APS has a specific order for the symbols; they are described in the order of  * † ‡ §. If the symbols are out of order or if other symbols have been used within the table, then you will have to reorder or alter them. If fewer than 4 symbols have been used, then change to letters (in alphabetical order).

%%%%% RQ1 and RQ2

Next, we verify if the search engines return biased results in terms of document stances (RQ1) and if so, we further investigate if the engines suffer from the same level of bias (RQ2) that the difference between the engines are not statistically significant. 
%
%For this, we computed MB and MAB scores for all three evaluation measures. 
%
In Table~\ref{tab:stance} %we observe that
all MB scores are positive and regarding the RQ1, the engines seem to be biased towards the pro stance. 
%the engines seem to be biased towards the pro stance (all MB scores are positive - RQ1). This means that both search engines are biased towards the same stance (RQ2).
%
We applied the one-sample t-test on MB scores to check the existence of stance bias, i.e. if the true mean is different from zero, as mentioned in Section~\ref{sec:protocol}. However, these biases are statistically not significant which means that this expectation may be the result of noise -- there is not a systematic stance bias, i.e. preference of one stance with respect to the other. 
%
Based on MAB scores, we can observe that both engines suffer from an absolute bias. However, the difference between the two engines is shown to be non-significant with the two-tailed t-test. %This bias is significant for all evaluation measures. 
%shows the p-values for both experiments all three evaluation measures of MB and MAB give consistent results. 
%
These results show that both search engines are not biased towards a \emph{specific} stance in returning results since there is no statistically significant difference from the \emph{ideal} distribution. Nonetheless, for both engines there exists an absolute bias which can be interpreted as the expected bias for a topic question. These empirical findings imply that the search engines are biased for some topics towards the pro stance and for others towards the against stance.
%Yet, all the three measures of MB (denoted as $\ast$).

%
The results are displayed in Figure~\ref{fig:dcgstance}. This figure refers to the values used to compute the MAB score of the DCG$@10$ column. %scores distribution of each query referring to the Table~\ref{tab:stance} and 
%
It shows that the difference between the pro and against stances of both engines for topics is uniformly distributed. To note that, no topic can be located on the up-right area of the plot because the sum of their coordinates is bounded by the maximum possible DCG$@10$ score. Moreover we observe that topics are distributed similarly across the engines.
%
This is also confirmed by Figure~\ref{fig:dcgdiffstance} where we can observe that the stance bias scores ($\beta_{DCG@10}$), i.e. the differences between DCG$@10$ scores for the pro stance and DCG$@10$ scores for the against stance, of topics are somehow balanced between the up-right quadrant and the low-left quadrant. Moreover, these two quadrants are the area of agreement in stance between the two engines. The other two quadrants contain those topics where the engines disagree. Here we can conclude that the engines agree with each other in the majority of cases.

%engine 1 and engine 2 are denoted as points. 
%
%We also put a line of equality ($y=x$) (i.e. Bing and Google scores for 
%The specified measures for the axis labels are \emph{equal} if they appear on the line) for comparison. 
%If a point lies above the line, this means that the 
%Google 
%y-axis label score of the corresponding query is higher than x-axis, and vice-versa. 
%
%The up-right (I: +/+) and low-left (III: -/-) regions have some points (the engines agree on the pro (+) and against (-) stances), while the up-left (IV: -/+) and low-right (II: +/-) have fewer points (the engines disagreed on) that the search engines mostly agree with each other. 
%

%%%%% RQ3
Lastly, we investigate if the search engines are biased in the ideology space (RQ3).
%
Looking at MB scores in Table~\ref{tab:political} we observe that both search engines seem to be biased towards the same ideological leaning -- liberal (all MB scores are negative). Unlike the stance bias, one sample t-test on MB scores show that these expectations are statistically significant with different confidence values, i.e. p-value < 0.005 across all three IR measures for engine 2; whereas the same confidence value on P$@10$ for engine 1 and p-value < 0.05 on RBP and DCG$@10$. These results indicate that both search engines are biased towards the same leaning which is liberal.
%the p-values for two aggregating measures of bias in terms of political perspective.
Comparing the two search engines on MB scores, we observe that their differences are statistically not significant, which means that the observed difference may be the result of random noise.
%
%However, the results are significant and all evaluation measures agreed on the fact that both search engines are \textit{biased}. 
%
%However, they are \textit{biased} as much since the difference between their bias scores (MB) of all three IR-based measures are non-significant. 
%
Based on MAB, since all MAB scores are positive we can also observe that both engines suffer from an absolute bias. However, in contrast with what observed for the stance bias, this time there is a difference in expected ideological bias between the two search engines. For RBP and DCG@10 the difference between the engines is statistically significant. This finding and the different user models that these evaluation measures model suggest that the perceived bias by the users may change based on their behaviour. A user that always inspects the first 10 results (as modelled by P$@10$) may perceive the same ideological bias between engine 1 and engine 2, while a less systematic user, which just inspects the top results, may perceive that engine 1 is more biased than engine 2. Moreover, comparing this finding with the performance of the engines, we can observe that the better performing engine is more biased than the worse performing one.

%On the other hand, there is a significant difference between the SERPs of engine 1 and engine 2 in terms of absolute bias (MAB), if we include strong concept of ranking in our analysis (i.e., with DCG and RBP measures), that Engine 1 is more \textit{biased}. 



%where the difference is non-significant for {\color{red}delta bias} but the difference both search engines are \textit{biased} and they are \textit{biased} as much in terms of political leanings if we include rank into our analysis. Moreover, our results show that Engine 1 (Bing) is more \textit{biased} and are significant with 95\% confidence (i.e., $\alpha = 0.05$). all evaluation measures also agreed on the fact that the two search engines have similar expected stance towards the same controversial topic because there is no significant difference between the SERPs of Bing and Google.

%Hence, we argue that both search engines tend to show biased results with respect to the controversial topics, and they tend to be biased in the same way. 

%In order to further compare the SERPs of the two search engines in stance and political perspective detection, 
%bias present in the two search engines, que
%we plotted the DCG and Diff DCG scores
%three sentiment-based metric scores 
%of all controversial queries in $\set{Q}$ to visualize the distribution of the values for Bing and Google in Figure~\ref{fig:dcgstance}, 
%Figure~\ref{fig:dcgdiffstance}, 
%Figure~\ref{fig:dcgpol}, and 
%Figure~\ref{fig:dcgdiffpol}. 
%
%We represented each query as a point; each point is a topic. 
%

Comparing Figure~\ref{fig:dcgpol} with Figure~\ref{fig:dcgstance} we observe that in Figure \ref{fig:dcgpol} the points look less uniformly distributed than in Figure \ref{fig:dcgstance}. Topics are mostly on the liberal side. Moreover, engine 2 has fewer points on the conservative side than engine 1. %shows the stance analysis per topic with the qcuery points of engine 1 and engine 2 which compare the DCG scores of two different stances as \emph{pro} and \emph{against}. 
%
%If a point lies above the line, this means that the \emph{against}-DCG score is higher than \emph{pro}-DCG for the corresponding query
%
%he following plots can be interpreted in a similar way.
Comparing Figure~\ref{fig:dcgdiffpol} with Figure~\ref{fig:dcgdiffstance}, we observe that the engines in Figure~\ref{fig:dcgdiffpol} are more biased towards the liberal side with respect to what observed in Figure~\ref{fig:dcgdiffstance}. Also, we observe that the engines mostly agree -- most of the points are placed on the up-right and low-left quadrants.

In conclusion, we find important to point out that it is not in the scope of this work to find the source of bias. As discussed in the introduction, bias may be a result of the input data, which may contain biases, or the search algorithm, which contains sophisticated features and specifically chosen algorithms that, although designed to be effective in satisfying information needs, may produce systematic biases. 
Nonetheless, we look at the problem from the user perspective and no matter where the bias comes from; the results are biased as described. Our findings seem to be consistent with prior works~\citep{robertson2017auditing, diakopoulos2018vote} that there exists liberal (left-leaning) partisan bias in SERPs; even in unpersonalised search settings~\citep{robertson2018auditing}. %Moreover, Epstein recently published a testimony~\citep{epsteingoogle} for the US Congress and based on the extensive experiments he has fulfilled so far, he stated that Google censored conservative content which legitimises Mr. Trump's argument.


\begin{comment}
\begin{figure*}
\centering
\begin{minipage}{.4\linewidth}
    \centering
    %\hspace{-1.8em}
    {\includegraphics[width=84mm,trim={2.5cm 6.5cm 4.5cm 6.5cm},clip]{figures/Stance_DCG.pdf}}
    \caption{$DCG_{\lps}@10$ against $DCG_{\las}@10$ measured on stances. Black points for engine 1 and yellow points for engine 2.}
    \label{fig:dcgstance}
\end{minipage}%
%\hspace{3em}
\begin{minipage}{.4\linewidth}
    \centering
    %\hspace{-1.8em}
    \includegraphics[width=84mm,trim={2.5cm 6.5cm 4.5cm 6.5cm},clip]{figures/Political_DCG.pdf}
    \caption{$DCG_\lcp@10$ against {$DCG_\llp@10$} measured on political perspectives. Black points for engine 1 and yellow points for engine 2.}
    \label{fig:dcgpol}
\end{minipage}%
%\vspace{0.3em}
\end{figure*}

\begin{figure*}
\centering
\hspace{-1.8em}
\begin{minipage}{.4\linewidth}
  \centering
    %\hspace{-1em}
    \includegraphics[width=84mm,trim={2.5cm 5.25cm 2cm 5cm},clip]{figures/Stance_Delta_DCG.pdf}
    \caption{$\beta_{DCG@10}$ measure}
    \label{fig:dcgdiffstance}
\end{minipage}
\hspace{3em}
\begin{minipage}{.4\linewidth}
    \centering
    \hspace{-1.8em}
    {\includegraphics[width=84mm],trim={2.5cm 5.25cm 2cm 5cm},clip]{figures/Political_Delta_DCG.pdf}}
    \caption{$\beta_{DCG@10}$ measured on perspectives, where positive is and negative is .}
    \label{fig:dcgdiffpol}
\end{minipage}
%vspace{0.3em}
\end{figure*}
\end{comment}


%depict political leaning analyses per topic. 
%
%Figure~\ref{fig:dcgpol} is akin to the Figure~\ref{fig:dcgstance}, the only difference is the axis labels which are transformed from
%\emph{pro-to-against} scale into the %\emph{conservative-to-liberal} scale. 
%
%Based on this observation, in Figure~\ref{fig:dcgpol} there are more points (queries) towards the \emph{liberal} (i.e., more points are above the line). 
%
%If we interpret the Figure~\ref{fig:dcgdiffpol} similarly to the Figure~\ref{fig:dcgpol} in terms of political perspectives, the points are mostly on the low-left (III: -/-) region (the engines mostly agree on \emph{liberal} (-)), which means they are more liberal as shown in Table~\ref{tab:political}.
%{\color{red} Based on this, the number of queries in total that Bing (Google) assigns higher scores are displayed on the x-axis (y-axis) label with percentage information.} 
%Moreover, in legend of these plots, we showed the linear coefficient $\rho$ values for each metric. 
%It can be seen that according to the $\text{B}_{P@10}$ metric, which does not consider the ranks of the retrieved documents, the search engines perform more similar (i.e. they are more correlated in terms of $\rho$ values) to each other as compared to the $\text{B}_{RBP}$ and $\text{B}_{DCG}$ measures. This suggests that the two search engines seem to be ranking the documents with the two different viewpoints {\color{red} (even though the differences in the mean value of the $B_{RBP}$ and \(NDCG_{Senti}\) metrics are not statistically significant).} 

%{\color{red}
%\subsubsection{Only non-polar controversial queries - Political Bias}

%ADD PLOT

%We also performed experiments to see the effect of the queries with inherent sentiment. As described in Section~\ref{DatasetCrawling}, we removed any queries that may be  polarized from the query set \(Q\), resulting in a query set \(Q_{nonPol}\) consisting of 53 queries that are not polarized. Table~\ref{table:nonPolar} shows the result of this experiment, which seem similar to the conclusions reached using all queries: The SERPs of both Bing and Google are \emph{biased}, but they have similar attitudes towards the same queries. However, different than the experiments of \emph{all} queries \(Q\), according to the \(AVG_{Senti}\) metric, Bing is not \emph{biased} while Google is still \emph{biased} with 99\% confidence. If we change the significance level of the t-test by setting $\alpha= 0.05$ (95\% confidence), then Bing becomes \emph{biased} as well. This suggests that results retrieved by Google may be slightly more biased than Bing, while the difference is not very big. }

==> limitations.tex <==

This work has potential limitations. As stated in the introduction, we focus on a particular kind of bias, known as \emph{statistical parity}, or more generally known as \emph{equality of outcome} instead of \emph{equality of opportunity} which uses query-specific base rates. In the context of the controversial topics where the document labels were obtained via crowd-sourcing, this bias measure, i.e. requiring equal representation of stances instead of query-specific base rates, made our experiments feasible. %Then, our choice of ideal ranking requires equal representation of stances instead of query-specific base rates which made our experiments feasible. 
This is firstly because, not all of the query questions in our list have certain answers based on scientific facts, i.e. some of them are subjective queries.
In investigating the equality of opportunity, queries can be further categorized as subjective and objective on top of our evaluation framework. For the objective queries, expert labels can be obtained and used as base rates, then search results can be evaluated by taking into account these base rates. Please note that our evaluation framework could better be applied to the controversial queries from the public's perspective mainly where the goal is to have balanced SERPs instead of skewed results. We believe that some queries should be handled with a different framework since those queries are not intrinsically controversial such as \emph{Is Holocaust real?} - there is only one correct answer without the need of a discussion.
%

Besides, the identification of the stance for the full ranking list is currently too expensive to get annotated via crowd-sourcing. To tackle this issue, a machine learning model can help us to automate the process of obtaining the stance labels. 
Another potential limitation is that some queries may not be real user queries. Nonetheless, we extracted the queries directly from their topic pages of the ProCon.org~\citeyearpar{ProCon} along with the topics. We deliberately did not change the queries to avoid any interference/bias from our side on the results. 
In this work, we did not make a domain-specific selection of the topics, or apply any filtering as subjective/objective, rather we accepted them as \emph{controversial} topics from the general public's perspective which is the main scope of this work.
%

Apart from these, crowd-workers' own personal biases may affect the labelling process. For this reason, we tried to mitigate these biases by i. asking the workers to annotate stances rather than ideologies to make their judgment more objective, and ii. aggregating the final judgment coming from multiple workers.
Additionally, our analysis refers to a specific point in time where the data was collected. To enable reproducibility and an easier comparison of these results at some point in the future, we made our dataset publicly available. %The bias analysis allows us to investigate bias in search results.
Lastly, we note that this bias analysis can only be used as an indicator of potentially biased ranking algorithms because it is not enough in order to track the source of bias. In the scope of this work, we did not investigate the source of bias that may come from the data (input bias) or from the ranking mechanism (algorithmic bias) of the corresponding search engines. 
Despite these potential limitations, we believe that our work is a good attempt to evaluate bias in search results with new bias measures and a dataset crawled specifically for the search bias evaluation. Since the bias analysis is very complex, we deliberately limited our scope and only focused on the bias analysis of \emph{recent} controversial topics in \emph{news} search. Nonetheless, all these limitations lead us to numerous interesting future directions.


%

==> notation.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu


Follows a set of symbols, functions, and labels used in this paper:
%\vspace{1.5em}

\begin{comment}
\begin{supertabular}{ l l }
\hline
\hline
{Symbols}\\
\hline
\hline
$\sS$   & set of search engines. \\
$s$     & a search engine $s \in \sS$. \\
$\sQ$   & set of queries. \\
$q$     & a query $q \in \sQ$. \\
%$d$     & a document. \\
$r$     & a SERP (a retrieved document). \\%(list of documents).
$r_i$   & the document in $r$ retrieved at rank $i$.\\
$|r|$   & size of $r = [r_1, r_2, \dots, r_{|r|}]$.\\
$n$     & number of documents considered in $r$ by $f$ (cut-off).\\
$G$     & a set of groups $g_i$ ($g_1 \cup g_2 \cup \dots \cup g_n = G$). \\
$g_i$   & a group $g_i \in G$. \\ \hline
%\hline
\hline
{Functions}\\
\hline
\hline
$s(q)$                  & returns $r$ given a query ($q$). \\ 
$j(r_i)$                & returns the label associated to $r_i$.\\
$j(q)$                  & returns the label associated to $q$.\\
$f(r)$                  & an evaluation measure for SERPs.\\
$f_g(r)$                & like $f$ but for $g$.\\
%$f_{-}(r)$             & like $f$ but for the against label.\\
$[\text{Condition}]$    & returns 1 if the condition is true and 0 otherwise.\\
\hline
\hline
{Labels}\\
\hline
\hline
$g_1$  & protected group. \\
$g_2$  & unprotected group. \\ \hline
$\lps$ & pro stance. \\
$\lns$ & neutral stance. \\
$\las$ & against stance. \\ 
$\lnr$ & not-relevant stance. \\ \hline
$\lcp$ & conservative political perspective.
\\
%$\lnp$ & neutral political perspective. \\
$\llp$ & liberal political perspective. \\
$\lbp$ & both or neither political perspectives. \\
%$+$ & label  .\\
%$-$ & against label.\\
\hline
\hline
\end{supertabular}
\end{comment}
%\end{center}
%\end{table}

==> related_work.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu


In recent years, bias analysis in SERPs of search engines has attracted a lot of interest~\citep{baeza2016data,mowshowitz2002bias,noble2018algorithms,pan2007google,tavani2012search} due to the concerns that search engines may manipulate the search results influencing users. The main reason behind these concerns is that search engines have become the fundamental source of information~\citep{dutton2013cultures}, and surveys from Pew~\citeyearpar{american2014personal} and Reuters~\citeyearpar{newman2018reuters} found that more people obtain their news from search engines than social media. The users reported higher trust on search engines for the accuracy of information~\citep{newman2018reuters, newman2019reuters, PewTrust} and many internet-using US adults even use search engines to fact-check information~\citep{dutton2017search}. 

To figure out how this growing usage of search engines and trust in them might have undesirable effects on public, and what could be the methods to measure those effects, in the following we review the research areas related first to automatic stance detection, then to fair ranking evaluation, and lastly to search bias quantification.

%\subsection{Opinion Mining} %Topic Discovery \& Sentiment Analysis}

\subsection{Opinion Mining and Sentiment Analysis}

A form of Opinion Mining related to our work is Contrastive Opinion Modeling (COM). Proposed by~\citet{fang2012mining}, in COM, given a political text collection, the task is to present the opinions of the distinct perspectives on a given query topic and to quantify their differences with an unsupervised topic model. COM is applied on debate records and headline news. Differently from keyword analysis to differentiate opinions using topic modelling, we compute different IR metrics from the content of the news articles to evaluate and compare the bias in the SERPs of two search engines. 
\citet{aktolga2013sentiment} consider the sentiment towards controversial topics and propose different diversification methods based on the topic sentiment. Their main aim is to diversify the retrieved results of a search engine according to various sentiment biases in blog posts rather than measure bias in the SERPs of~\emph{news} search engines as we do in this work.

\citet{demartini2010dear} exploit automatic and lexicon-based text classification approaches, Support Vector Machines and SentiWordNet respectively to extract sentiment value from the textual content of SERPs in response to controversial topics. %Then, only this sentiment information is used to detect and compare opinions in the retrieved results of three commercial search engines without measuring bias as we present in this study.
Unlike us,~\cite{demartini2010dear} only use this sentiment information to compare opinions in the retrieved results of three commercial search engines without measuring bias.
In this paper, we propose a new bias evaluation framework with robust bias measures to systematically measure bias in SERPs. 
\citet{chelaru2012querysent} focus on queries rather than SERPs and investigate if the opinionated queries are issued to search engines by computing the sentiment of suggested queries for controversial topics. In a follow-up work \citep{chelaru2013querysentfollow}, authors use different classifiers to detect the sentiment expressed in queries and extend the previous experiments with two different use cases. %Since our work analyses the SERPs and focuses on the news domain, we identify the stance of the news articles towards a topic via crowd-sourcing. %In our work, we use opinion mining to detect different viewpoints in SERPs in order to quantify bias.
Instead of queries, our work analyses the SERPs in~\emph{news} domain, therefore we need to identify the stance of the news articles. Automatically obtaining article stances is beyond the scope of this work, thus we use crowd-sourcing.
%Since  instead of queries, Our work analyses the news SERPs instead of queries, therefore to identify the stance of the news articles we use crowd-sourcing 

%Queries may contain inherent polarity as SERPs do. According to~\cite{koutra2015events}, users tend to phrase queries in a way that confirms their own beliefs such as ``Obama born in kenya''. Moreover, selected keywords in a query may imply a perspective as in ``gun control'' vs. ``gun rights''. Therefore, we experimented with and without \emph{polarized} queries in our query set.

\subsection{Evaluating Fairness in Ranking}
\label{subsec:fairness_evaluation}
Fairness evaluation in ranked results has attracted attention in recent years.
\citet{yang2017measuring} propose three bias measures, namely Normalized discounted difference (rND), Normalized discounted Kullback-Leibler divergence (rKL) and Normalized discounted ratio (rRD) that are related to Normalized Discounted Cumulative Gain (NDCG) through the use of logarithmic discounting for regularization which is inspired from NDCG as also stated in the original paper.
%for ranked outputs to quantify fairness 
%in a ranking scheme %Moreover, a data generation procedure is developed to systematically control the degree of unfairness in the output and evaluate the proposed measures. % on synthetically generated and the real datasets.
%In this fairness quantification framework, 
Researchers use these metrics to check if there exists a systematic discrimination against a group of individuals, when there are only two different groups as a protected ($g_1$) and an unprotected group ($g_2$) in a ranking. In other words, researchers quantify the relative representation of $g_1$ (the protected group), whose members share a characteristic such as race or gender that cannot be used for discrimination, in a ranked output.
%These proposed measures have the following shape: %For example, rND is defined as follows:
The definitions of these three proposed measures can be rewritten as follows:
%
\begin{linenomath*}
\begin{equation}
\label{eq:yang_1}
    f_{g_1}(r) = \frac{1}{Z} \sum_{i=10, 20, \dots}^{|r|}
    \frac{1}{\log_2i}%{\log_2(i+1)}
    \left|d_{g_1}(i,r)\right|,
\end{equation}
\end{linenomath*}
%
where $f(r)$ is a general definition of an evaluation measure for a given ranked list of documents, i.e. a SERP, whereas $f_{g_1}$ is specifically for the protected group of $g_1$. In this definition, $Z$ is a normalisation constant, $r$ is the ranked list of the retrieved SERP and $|r|$ is the size of this ranked list, i.e. number of documents in the ranked list. 
Note that, $i$ is deliberately incremented by 10, to compute \emph{set-based fairness} at discrete values as top-10, top-20 etc., instead of 1 as usually done in IR for the proposed measures to show the correct behaviour with bigger sample sizes. The purpose of computing the~\emph{set-based fairness} to express that being fair at higher positions of the ranked list is more important, e.g. top-10 vs. top-100.

%
In the rewritten formula, $d_{g_1}$ defines a distance function between the expected probability to retrieve a document belonging to $g_1$, i.e. in the overall population, and its observed probability at rank $i$ to measure the systematic bias. These probabilities turn out to be equal to P@n:
%
\begin{linenomath*}
\begin{equation}\label{eq:pc}
    \text{P}_{g_1}@n=\frac{1}{n}\sum_{i=1}^n[j(r_i) = g_1],
\end{equation}
\end{linenomath*}
%
when computed over $g_1$ at cut-off value $|r|$ and $i$ for the three proposed measures as below. In this formula, $n$ is the number of documents considered in $r$ as a cut-off value, and $r_i$ is defined as the document in $r$ retrieved at rank $i$. Note that, $j(r_i)$ returns the label associated to the document $r_i$ specifying its group as $g_1$ or $g_2$. Based on this, $[j(r_i) = g_1]$ refers to a conditional statement which returns 1 if the document $r_i$ is the member of $g_1$ and 0 otherwise.
%
%where $d(i, r)$ represents a distance between the input distribution we find at rank $i$ and the expected distribution in the collection of documents. 
%
\noindent In the original paper, $d_{g_1}$ is defined for %{\color{red} add the full names of these measures} 
rND, rKL, and rRD as:

%
\begin{linenomath*}
\begin{align}
    d_{g_1}(i,r) = & \text{P}_{g_1}@i - \text{P}_{g_1}@{|r|} \; & \text{for rND},\\
    d_{g_1}(i,r) = & - \text{P}_{g_1}@i \log \left(\frac{\text{P}_{g_1}@{|r|}}{\text{P}_{g_1}@i}\right) \\ 
    & \qquad - (1-\text{P}_{g_1}@i) \log \left(\frac{1-\text{P}_{g_1}@{|r|}}{1-\text{P}_{g_1}@i}\right) \; & \text{for rKL},\\
    d_{g_1}(i,r) = & \frac{\text{P}_{g_1}@i}{1-\text{P}_{g_1}@i} - \frac{\text{P}_{g_1}@{|r|}}{1-\text{P}_{g_1}@{|r|}} \; & \text{for rRD}.
\end{align}
\end{linenomath*}
%
\\\\

These measures, although inspired by IR evaluation measures, particularly in the context of content bias in search results suffer from the following limitations:
\begin{enumerate}
\item rND measure focuses on the protected group ($g_1$). If we were to compute $f$ at steps of $1$ with the given equal desired proportion of the two groups as 50:50, then the distance function of rND, denoted as $d_{g_1}$ would always give a value of 0.5 for the first retrieved document, where $i=1$. This will always be the case, no matter which group this document belongs to, e.g. \emph{pro} or \emph{against} in our case. This is caused by $d_{g_1}$ of rND through the use of its absolute value in Eq.~\eqref{eq:yang_1}. In our case, this holds when $i=1, 2, 4$ and $r = 10$ where we measure bias in the top-10 results. This is in fact avoided in the original paper~\citep{yang2017measuring} by computing $f$ at steps of $10$ as top-10, top-20 etc. rather than the steps of $1$ as it is usually done in IR which gives more meaningful results in our evaluation framework.
%

\item rKL measure cannot differentiate between biases of equal magnitude, but in opposite directions with the given equal desired proportion of the two groups as 50:50, i.e. it cannot differentiate bias towards \emph{conservative}, or \emph{liberal} in our case. Also, in IR settings it is not as easy to interpret the computed values from the KL-divergence (denoted as $d_{g_1}$ for rKL) compared to our measures since our measures are based on the standard utility-based IR measures. %which directly compute the bias values per document in top-10 of the search results for search bias evaluation. 
Furthermore, KL-divergence tends to generate larger distances for small datasets, thus it could compute larger bias values in the case of only $10$ documents, and this situation may become even more problematic if we measure bias for less number of documents, e.g. top-3, top-5 for a more fine-grained analysis. In the original paper, this disadvantage is alleviated by computing the rKL values also at discrete points of steps $10$ instead of $1$.

%
\item rRD measure does not treat the protected and unprotected groups ($g_1$ and $g_2$) symmetrically as stated in the original paper, which is not applicable to our framework. Our proposed measures treat $g_1$ and $g_2$ equal since we have two protected groups; \emph{pro} and \emph{against} for stance bias, \emph{conservative} and \emph{liberal} for ideological bias to measure bias in search settings. Moreover, rRD is only applicable in special conditions when $g_1$ is the minority group in the underlying population as also declared by the authors, while we do not have such constraints for our measures in the scope of search bias evaluation.

%
\item These measures focus on differences in the relative representation of $g_1$ between distributions. Therefore, from a general point of view, most probably more samples are necessary for these measures to show the expected behavior and work properly. In the original paper, experiments are fulfilled with three different datasets, one is synthetic which includes 1000 samples and two are real datasets which include 1000 and 7000 samples to evaluate bias with these measures, while we have only 10 samples for query-wise evaluation. This is probably because these measures were mainly devised for the purpose of measuring bias in ranked outputs instead of search engine results; none of these datasets contain search results either. 
%
\item These measures are difficult to use in practice, since they rely on a normalization term, $Z$ that is computed stochastically, i.e. as the highest possible value of the corresponding bias measure for the given number of documents $n$ and protected group size |$g_1$|. In this paper, we rely on standard statistical tests, since they are easier to interpret, provide confidence intervals, and have been successfully used to investigate inequalities in search systems previously by~\citet{chen2018investigating}.
%
\item These measures do not consider relevance which is a fundamental aspect when evaluating bias in search engines. For example, as in our case, when searching for a controversial topic, if the first retrieved document is about a news belonging to $g_1$ but its content is not relevant to the searched topic, then these measures would still consider this document as positive for $g_1$. However, this document has absolutely no effect on providing an unbiased representation of the controversial topic to the user. This is because these metrics were devised particularly for evaluating bias in the ranked outputs instead of SERPs.
\end{enumerate}
Although the proposed measures by~\citet{yang2017measuring} are valuable in the context of measuring bias in ranked outputs where the individuals are being ranked and some of these individuals are the members of the protected group ($g_1$), these measures have the aforementioned limitations. These limitations are particularly visible for content bias evaluation where the web documents are being ranked by search engines in a typical IR setting. In this paper we address these limitations by proposing a family of fairness-aware measures with the main purpose of evaluating content bias in SERPs, based on standard utility-based IR evaluation measures.
\\
\indent\citet{zehlike2017fa}, based on \citet{yang2017measuring}'s work, %aim to achieve statistical parity in ranked output through connecting the creation of ranking with assessing fairness metrics. 
propose an algorithm to test the statistical significance of a fair ranking.
%
\citet{beutel2019fairness} propose a pairwise fairness measure for recommender systems. %Similarly to our work the authors follow the equality of opportunity principle by \cite{hardt2016equality}. 
%Nonetheless, their primary focus is on under-recommended items, whereas we do not focus on a specific group. 
However, the authors, unlike us, measure fairness on personalized recommendations and %but we work in an unpersonalized information retrieval setting and unlike us they also 
do not consider relevance, while we work in an unpersonalized information retrieval setting and we do consider relevance. % labels are known for each item in a ranking.
%
%\citet{kallus2019fairness} studies the cross-ROC curve and the corresponding xAUC metric for auditing disparities in a bipartite ranking setting, which is described as finding a good ranking function to rank positively labeled examples above negative ones. Unlike \cite{kallus2019fairness}, %which focuses on the bipartite ranking setting where the AUC loss mainly evaluates the ranking quality of the entire distribution, our method is concerned with measuring fairness in a search engine by analyzing a fair representation of a political perspective in SERPs.% and our proposed metrics such as DCG-based and top-k metrics evaluate only a portion of the distribution, i.e., returned ranked documents, to detect bias.
\citet{kallus2019fairness} investigate the fairness of predictive risk scores as a bipartite ranking task, where the main goal is to rank positively labelled examples above negative ones. 
%Whilst, in this paper we aim to measure fairness in ranking % as an information retrieval application, i.e., 
%in terms of fair representation in SERPs, instead of the bipartite ranking setting. 
However, their measures of bias based on the area under the ROC curve (AUC) are agnostic from the rank position at which a document has been retrieved. %DCG-based and top-k measures, which emphasize the position of an item in a portion of the search results, the researchers in \cite{kallus2019fairness} present an AUC-variant metric that focuses on ranking quality of the entire search result.
%the synthetic ranking generation procedure of \cite{yang2017measuring} is used to calibrate the proposed algorithm, FA*IR, and optimize the utility of a ranking. The focus of \cite{zehlike2017fa}


%In our work, we do not require the generation of \emph{randomized ranking}, therefore not relying on any other search engine. 

%The work proposed by~\citet{demartini2010dear} can be considered as relevant to ours since supervised and lexicon-based text classification techniques were exploited to detect document and sentence-level sentiment in the textual content where the authors analysed 14 controversial queries for three search engines. However, different from our work, their aim is not to measure bias, but to compare the opinions represented in the SERPs using only average sentiment scores and visualisation.


\subsection{Quantifying Search Engine Biases}
Although the search engine algorithms are not transparent and available to external researchers, algorithm auditing techniques provide an effective means for systematically evaluating the results in a controlled environment~\citep{sandvig2014auditing}.
Prior works leverage LDA-variant unsupervised methods and crowd-sourcing to analyse bias in content, or URL analysis for indexical bias.



%Researchers quantify bias (partisanship) in US news outlets (newspapers and 2 political blogs) for 15 selected queries related to a wide range of controversial issues about which Democrats and Republicans argue. They used a combination of machine-learning and crowdsourcing techniques for content-based analysis. 
%***"Finally, news organizations express their ideological bias not by directly advocating for a preferred political party, but rather by disproportionately criticizing one side, a convention that further moderates overall differences." (Interesting)
%Articles are represented with 1000-dimensional vector and for the labels of them they used AMT for the news and politics classifiers. Quantifying bias için crowdsourcing'i ilk defa bu ekip kullanıyor. Hem topic (LDA den alınan suggested two topics) hem de ideological slant'lerini AMT'de label'latıyorlar bir sample'ın.
%Daha önce audience-based ve content-based bias çalışmaları vardı. Ama audience-based provides only relative not absoulute measures of slant. Bunlar da "content-based" yapıyorlar eğer ikiye ayırırsak yoksa aslında rater-based yapıyorlar content-based altında crowdsourcing kullandıkları için.
%Result: They found that US news outlets are substantially more similar fro lect to right-and less partisan-than generally believed. No strong liberal bias exists in the US media.
%\textcolor{red}{Check here}

%First: Content analyis 
%i.LDA-variant unsupervised methods
\citet{saez2013social} propose unsupervised methods to characterise different types of biases in online news media and in their social media communities by also analysing political perspectives of the news sources.
\citet{yigit2016towards} investigate media bias by analysing the user comments along with the content of the online news articles to identify the latent aspects of two highly polarising topics in the Turkish political arena. \citet{kulshrestha2017quantifying} quantify bias in social media by measuring the bias of the author of a tweet, while in \citet{kulshrestha2018search}, bias in web search is quantified through a URL analysis for Google in political domain without any SERP content analysis. In our work, we consider the Google and Bing SERPs from news sources such as NY-Times, and BBC news in order to quantify bias through content analysis.

%ii.Crowd-sourcing
In addition to the unsupervised approaches, crowd-sourcing is a widely used mechanism to analyse bias in content.
Crowd-sourcing is a common approach for labelling tasks in different research areas such as image \& video annotation \citep{crowd-image,crowd-video}, object detection \citep{crowd-object}, named entity recognition \citep{crowd-ner,crowd-twitter}, sentiment analysis \citep{crowd-sentiment} and relevance evaluation \citep{crowd-relevance, crowd-trec}. \citet{crowd-survey} provide a detailed survey of crowd-sourcing applications. As \citet{crowd-survey} suggest, crowd-sourcing can also be used for gathering opinions from the crowd. \citet{crowd-opinion} use crowd-sourcing to classify Spanish consumer comments and show that non-expert Amazon Mechanical Turk (MTurk) annotations are viable and cost-effective alternative to expert ones. In this work, we use crowd-sourcing for collecting opinions of the public not about consumer products but controversial topics.

%Second: URL analysis for indexical bias
Apart from the content bias, there is another research area, namely indexical bias.
Indexical bias refers to the bias which is displayed in the selection of items, rather than in the content of retrieved documents, namely content bias \citep{mowshowitz2002bias}. \citet{mowshowitz2002assessing,mowshowitz2005measuring} quantify instead only indexical bias by using precision and recall measures. Moreover, the researchers approximate the \emph{ideal} (i.e. norm) by the distribution produced by a collection of search engines to measure bias. Yet, this may not be a \emph{fair} bias evaluation procedure since the \emph{ideal} itself should be \emph{unbiased}, whereas the SERPs of search engines may actually contain \emph{bias}. Similarly, \citet{chen2006position} use the same method in order to quantify indexical and content bias, however, content analysis was performed by representing the SERPs with a weighted vector with different HTML tags without an in-depth analysis of the textual content. In this work, we evaluate content bias by analysing the textual contents of the Google and Bing SERPs, and we do not generate the \emph{ideal} relying on the SERPs of other search engines in order to measure bias in a more \emph{fair} way.
%
In addition to the categorisation of the content and indexical bias analysis, prior methods used in auditing algorithms to quantify bias can also be divided into three main categories as \emph{audience-based}, \emph{content-based}, and \emph{rater-based}.
\emph{Audience-based} measures focus on identifying the political perspectives of media outlets and web pages by utilising the interests, ideologies, or political affiliations of its users, e.g., likes and shares on Facebook~\citep{bakshy2015exposure}, based on the premise that readers follow the news sources that are closest to their ideological point of view~\citep{mullainathan2005market}.~\citet{lahoti2018joint} model the problem of ideological leaning of social media users and media sources in the liberal-conservative ideology space on Twitter as a constrained non-negative matrix-factorisation problem.
\emph{Content-based} measures exploit linguistic features in textual content; \cite{gentzkow2010drives} extract frequent phrases of the different political partisans (Democrats, Republicans) from the Congress Reports. Then, the researchers come with the metric of media slant index to measure US newspapers' political leaning. Finally, rater-based methods also exploit textual content and can be evaluated under the content-based methods. Unlike the content-based, the \emph{rater-based} methods use ratings of people for the sentiment, partisan or ideological leaning of content instead of analysing the textual content linguistically. Rater-based methods generally leverage crowd-sourcing to collect the labels for the content analysis. For instance, \citet{budak2016fair} quantify bias (partisanship) in US news outlets (newspapers and 2 political blogs) for 15 selected queries related to a wide range of controversial issues about which Democrats and Republicans argue. The researchers use MTurk as a crowd-sourcing platform to obtain the topic and political slant labels, i.e. being positive towards Democrats or Republicans, of the articles. Similarly, \citet{robertson2017auditing} use crowd-sourcing to score individual search results and \cite{diakopoulos2018vote} make use of the MTurk platform, i.e. rater-based approach, to get labels for the Google SERP websites by focusing on the content and apply an audience-based approach through utilising the prior work of~\cite{bakshy2015exposure} specifically for quantifying partisan bias. Our work follows a rater-based approach by making use of the MTurk platform for crowd-sourcing to analyse web search bias through stances and ideological leanings of the news articles instead of partisan bias in the textual contents of the SERPs.

There have been endeavors to audit partisan bias on web search. %provide a beneficial tool and have previously been examined to quantify partisan bias.
%analyse the effect of personalisation and location on search rankings~\cite{kliman2015locationbasedsearch, hannak2013personalizedsearch}.
%Apart from these studies, there have been recent works to audit partisan bias in non-personalised web search. 
\citet{diakopoulos2018vote} present four case studies on Google search results and to quantify partisan bias in the first page, they collect SERPs by issuing complete candidate names of the 2016 US presidential election as queries and utilise crowd-sourcing to obtain the sentiment scores of the SERPs. They found that Google presented a higher proportion of negative articles for Republican candidates than the Democratic ones. Similarly, \citet{robertson2017auditing} present a case study for the election and use a browser extension to collect Google and Yahoo search data for the election-related queries, then use crowd-sourcing to score the SERPs. The researchers also found a left-leaning bias and Google was more biased than Yahoo. In their follow-up work, they found a small but significant ranking bias in the standard SERPs but not due to personalisation~\citep{robertson2018auditing}. Similarly, researchers audit Google search after Donald Trump's Presidential inauguration with a dynamic set of political queries using auto-complete suggestions~\citep{robertson2018political}.~\citet{hu2019auditing} conduct an algorithm audit and construct a specific lexicon of partisan cues for  measuring political partisanship of Google Search snippets relative to the corresponding web pages. They  define the corresponding difference as bias for this particular use case without making a robust search bias evaluation of SERPs from the user's perspective. In this work, we introduce novel fairness-aware IR measures which involve rank information to evaluate content bias. For this, we use crowd-sourcing to obtain labels of the~\emph{news} SERPs returned towards the queries related to a wide-range of controversial topics instead of only political ones. With our robust bias evaluation measures, our main aim is to audit ideological bias in web search rather than solely partisan bias.

%
Apart from partisan bias, recent studies have investigated different types of bias for various purposes.~\citet{chen2018investigating} investigate gender bias in the various resume search engines, which are platforms that help recruiters to search for suitable candidates and use statistical tests to examine two types of indirect discrimination: individual and group fairness.
Similarly in another research study, authors investigate gender stereotypes by analyzing the gender distribution in image search results retrieved by Bing in four different regions~\citep{otterbacher2017competent}. Researchers use the query of `person' and the queries related to 68 character traits such as `intelligent person', and the results show that photos of women are more often retrieved for `emotional' and similar traits, whereas `rational' and related traits are represented by photos of men. In a follow-up work, researchers conduct a controlled experiment via crowd-sourcing with participants from three different countries to detect bias in image search results~\citep{otterbacher2018investigating}. Demographic information along with measures of sexism are analysed together and the results confirm that sexist people are less likely to detect and report gender biases in the search results.

~\citet{raji2019actionable} examine the impact of publicly naming biased performance results of commercial AI products in face recognition for directly challenging companies to change their products.~\citet{geyik2019fairness} present a fairness-aware ranking framework to quantify bias with respect to protected attributes and improve the fairness for individuals without affecting the business metrics. 
The authors extended the metrics proposed by~\citet{yang2017measuring}, of which we specified the limitations in Section~\ref{subsec:fairness_evaluation}, and evaluated their procedure using simulations with application to LinkedIn Talent Search.~\citet{vincent2019measuring} measure the dependency of search engines on user-created content to respond to queries using Google search and Wikipedia articles. In another work, researchers propose a novel metric that involves users and their attention for auditing group fairness in ranked lists~\citep{sapiezynski2019quantifying}.~\citet{gao2019fair} propose a framework that effectively and efficiently estimate the solution space where fairness in IR is modelled as an optimisation problem with fairness constraint. Same researchers work on top-k diversity fairness ranking in terms of statistical parity and disparate impact fairness and propose entropy-based metrics to measure the topical diversity bias presented in SERPs of Google using clustering instead of a labelled dataset with group information~\citep{gao2020toward}. Unlike to their approach, our goal is to quantify search bias in SERPs rather than topical diversity. For this, we use a crowd-labelled dataset, thereby to evaluate bias from the user's perspective with stance and ideological leanings of the documents.

%In many works, fairness in IR is modelled as an optimisation problem with fairness constraint. For instance, 


%\textcolor{red}{TODO: 2018-2019 cite papers} \\

%
In this context, we focus on proposing a new search bias evaluation procedure in ranked lists to quantify bias in the~\emph{news} SERPs. With the proposed robust fairness-aware IR measures, we also compare the relative bias of 
%we also make a bias-wise comparison of 
the two search engines through incorporating relevance and ranking information into the procedure without tracking the source of bias as discussed in Section \ref{sec:introduction}. Our procedure can be used for the source of bias analysis as well which we leave as future work.
%Consequently, to propose a stronger claim about algorithmic bias, one needs to fulfill a two-phased analysis of i. evaluating bias on SERPs, and ii. tracking the source of bias. We propose  that may be used in both steps of the analysis and in the scope of this work, we implement the first part, which is a preliminary step for the second phase, i.e., investigating the source of bias, to be completed in the follow-up work.


==> results.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu


In Table \ref{tab:performance} we present the performance of the two search engines. This is measured over all the topics. A document is considered relevant when classified as pro, against, or neutral. The difference for all evaluation measures is statistically significant.

\begin{table*}[!t]
    \centering
    \caption{
    Stance bias of the search engines, p-values of a two-tailed \\ paired t-test computed between engine 1 and 2 
    %P-values of two-tailed paired t-test computer between engine 1 and 2.
    %$\ast$ indicates non statistical significance %while $\dag$ (p-value < 0.001) statistical significance 
    %of a one-sample t-test.
    }
    \begin{tabular}{cccccccc}
        \hline\hline
        & & P@10 & & RBP & & DCG@10 & \\
        \hline
        \multirow{3}{*}{MB} 
        & Engine 1 & 0.0281 && 0.0197 && 0.1069 &\\	
        & Engine 2 & 0.0175	&& 0.0271 && 0.1142 &\\
        \cline{2-8}
        & p-value & $>0.05$ & & $>0.05$ & & $>0.05$ & \\
        \hline
        \multirow{3}{*}{MAB} 
        & Engine 1 & 0.2596	&& 0.2738 &&	1.3380 &\\
        & Engine 2 & 0.2246 &&	0.2266 &&	1.0789 &\\
        \cline{2-8}
        & p-value & $>0.05$ & & $>0.05$ & & $>0.05$ & \\
        \hline\hline
    \end{tabular}
    \label{tab:stance}
\end{table*}

\begin{table*}[!t]
    \centering
    \caption{Ideological bias of the search engines, p-values of a two-tailed \\ paired t-test computed between engine 1 and 2 %P-values of two-tailed paired t-test. 
    %$\ddag$ (p-value < 0.005) and $\dag$ (p-value < 0.05) signify statistical significance on a one-sample t-test.
    }
    \hspace{-0.7em}\begin{tabular}{cccccccc}
        \hline\hline
        & & P@10 & & RBP & & DCG@10 & \\
        \hline
        \multirow{3}{*}{MB} 
        & Engine 1 & -0.1368 & & -0.1247 & & -0.6290 & \\	
        & Engine 2 & -0.1289 & & -0.1386 & & -0.6591 &\\
        \cline{2-8}
        & p-value & $>0.05$ & & $>0.05$ & & $>0.05$ &\\
        \hline
        \multirow{3}{*}{MAB} 
        & Engine 1 & 0.2579 && 0.2894 && 1.3989 & \\
        & Engine 2 & 0.2184	&& 0.2158 && 1.0456 &  \\
        \cline{2-8}
        & p-value & $>0.05$ & & $<0.05$ & & $<0.05$ \\
        \hline\hline
    \end{tabular}
    \label{tab:political}
    %\vspace{1.2em}
\end{table*}

In Table \ref{tab:stance} we present the stance bias of the search engines.
Note that for all the three measures of bias, P@10, RBP and DCG@10, lower value is better which means lower bias in the scope of this work as opposed to their corresponding classic IR measures.
All MB and MAB scores are positive for all three IR evaluation measures. %The one-sample t-test computed on MBs are non-statistically significant and denoted as (*). 
Also, the differences between the two search engines for both MB and MAB measures are statistically not significant and it is shown with the two-tailed pair t-test on these measures.
In Table \ref{tab:political} we show the ideological bias. Similarly to Table \ref{tab:stance}, lower is better since we use the same measures of bias.
This table is similar to Table \ref{tab:stance}. Unlike the Table \ref{tab:stance}, all MB scores are negative while all MAB scores are positive for all three IR evaluation measures. %The one-sample t-test computed on MBs are statistically significant for all the measures with different confidence values. 
The two-tailed paired t-test computed on MBs to compare the difference in bias between engine 1 and engine 2, this is statistically not significant. Nonetheless, the two-tailed test on MABs is statistically not significant for the measure P@10; but it is statistically significant for the measures RBP and DCG@10.

%for the measure of P@10 is non-statistically significant, whereas for the measures of RBP and DCG@10, it is statistically significant and denoted as ($\dag$). Also here when comparing the bias between engine 1 and engine 2 this is not statistically significant. However, when measuring the bias between engine 1 and engine 2 for the measures RBP and DCG@10, it is statistically significant. Moreover, the political bias measured by MAB is statistically significant on a one-sample t-test.



%left-lower-right-upper
\begin{figure}[!t]
\vspace{-1.2em}
\centering
%\hspace{-1.8em}
    \begin{minipage}{0.45\textwidth}
        \centering
        \vspace{0.6em}
        \includegraphics[width=\textwidth,trim={2.5cm 6.5cm 4.5cm 6.5cm},clip]{Stance_DCG.pdf}
        \caption{$DCG_{\lps}@10$ against $DCG_{\las}@10$ measured on stances -- black points for engine 1 and yellow points for engine 2}
        \label{fig:dcgstance}
\end{minipage}
\hspace{1.8em}
    \begin{minipage}{0.45\textwidth}
        \centering
        \vspace{1.4em}
        %\hspace{-1.8em}
        \includegraphics[width=\textwidth,trim={2.5cm 6.5cm 4.5cm 6.5cm},clip]{Political_DCG.pdf}
        \caption{$DCG_{\lcp}@10$ against $DCG_{\llp}@10$ measured on ideological leanings -- black points for engine 1 and yellow points for engine 2}
    \label{fig:dcgpol}
\end{minipage}
\vspace{2em}
\end{figure}

\begin{figure}[!t]
\centering
%\hspace{-1.8em}
\begin{minipage}{.43\textwidth}
  \centering
    %\hspace{-1em}
    \includegraphics[width=\textwidth,trim={2.5cm 5.25cm 2cm 5cm},clip]{Stance_Delta_DCG.pdf}
    \caption{$\beta_{DCG@10}$ measured on stances, where positive is $\lps$ and negative is $\las$}
    \label{fig:dcgdiffstance}
\end{minipage}
\hspace{2.8em}
\begin{minipage}{.43\textwidth}
    \centering
    \vspace{0.1em}
    %\hspace{-1em}
    {\includegraphics[width=1\textwidth,trim={2.5cm 5.25cm 2cm 5cm},clip]{Political_Delta_DCG.pdf}}
    \caption{$\beta_{DCG@10}$ measured on leanings, where positive is $\lcp$ and negative is $\llp$}
    \label{fig:dcgdiffpol}
\end{minipage}
%\vspace{-1.5em}
\end{figure}

In Figure \ref{fig:dcgstance} we show how the topic-wise SERPs distribute over the pro-against stance space for the measure DCG@10. The x-axis is the pro stance score ($DCG_{\lps}@10$) and the y-axis is the against stance score ($DCG_{\las}@10$). 
Each point corresponds to the overall SERP score of a topic. Black points are those SERPs retrieved by engine 1 and yellow points are those retrieved by engine 2.

In Figure \ref{fig:dcgdiffstance} we compare the overall stance bias score ($\beta_{DCG@10}$), i.e. difference between the pro and against stance scores, of SERPs for each topic measured on the two search engines. The x-axis is engine 1 and the y-axis is engine 2. The points in positive coordinates denote the topics whose SERPs are overall biased towards the pro stance, negative coordinates are for the against stance. 

Figure \ref{fig:dcgpol} and Figure \ref{fig:dcgdiffpol} are similar to Figure \ref{fig:dcgstance} and Figure \ref{fig:dcgdiffstance} but instead of measuring the stance bias we measure the ideological bias in the former case. Therefore, Figure \ref{fig:dcgpol} displays how the overall SERPs of topics distribute over the conservative-liberal ideological space for the measure DCG@10. Similarly, in Figure \ref{fig:dcgdiffpol} we compare the overall ideological bias score ($\beta_{DCG@10}$), i.e. difference between the conservative and liberal leaning scores, of the SERPs where the points in positive coordinates stand for the topics that are biased towards the conservative leaning, negative coordinates are for the liberal.

%\begin{figure}[!ht]
%\centering
%\captionsetup{justification=centering}
%    \includesvg[width=0.53\textwidth]{figures/AvgPol}
%    \captionsetup{font=scriptsize}
%   \caption[short]{The distribution of \textit{all} \\ queries on \(AVG_{Senti}@10\)}
%    \label{fig:avg}
%\end{figure}

%\begin{figure}[h!]
%    \begin{minipage}[t]{0.52\textwidth}
%    \includesvg[width=\textwidth]{figures/NDCG.svg}
%    \captionsetup{font=scriptsize}
%    \caption[short]{The distribution of \textit{all} \\ queries on \(NDCG_{Senti}@10\)}
%    \label{fig:ndcg}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[t]{0.5\textwidth}
%    \includesvg[width=\textwidth]{figures/AP.svg}
%    \captionsetup{font=scriptsize}
%    \caption[short]{The distribution of \textit{all} \\ queries on \(AP_{Senti}@10\)}
%    \label{fig:ap}
%    \end{minipage}
%\end{figure}

%{\color{red} Something about Q1}


==> search_bias_evaluation_framework.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu

In this section we describe our  search bias evaluation framework. Then, we present the measures of bias and the proposed protocol to identify search bias. %To begin with, a set of symbols, functions, and labels used throughout this paper can be found in Table~\ref{table:notation}.

\subsection{Preliminaries}
\label{sec:preliminaries}

Our first aim is to detect bias with respect to the distribution of stances expressed in the contents of the SERPs. % and the term \emph{sentiment polarity} reflects the emotion  in a given text.

%Follows a set of symbols, functions, and labels used in this paper:
%\vspace{1.5em}

Let $\set{S}$ be the set of search engines and $\set{Q}$ be the set of queries about controversial topics. 
When a query $q \in \set{Q}$ is issued to a search engine $s \in \set{S}$, the search engine $s$ returns a SERP $r$. 
We define the stance of the $i$-th retrieved document $r_i$ with respect to $q$ as $j(r_i)$. A stance can have the following values:
\emph{pro}, % ($+$), 
\emph{neutral}, % ($\cdot$), 
\emph{against}, % (-) or 
\emph{not-relevant}. % ($\times$).

A document stance with respect to a topic can be:
\begin{itemize}
\item\textbf{pro} ($\lps$) when the document is in favour of the controversial topic. The document describes more the pro aspects of the topic;
\item\textbf{neutral} ($\lns$) when the document does not support or help either side of the controversial topic. The document provides an impartial (fair) description about the pro and cons of the topic;
\item\textbf{against} ($\las$) when the document is against the controversial topic. The document describes more the cons aspects of the topic;
\item\textbf{not-relevant} ($\lnr$) when the document is not-relevant with respect to the controversial topic.
\end{itemize}

For our analyses, we deliberately use recent \emph{controversial} topics in US that are the real debatable ones rather than the topics being possibly exposed to false media balance, which occurs when the media present opposing viewpoints as being more equal than the evidence supports, e.g. Flat Earth debate~\citep{FalseBalance, FalseBalance2}. Our topic set contains abortion, illegal immigration, gay marriage, and similar \emph{controversial} topics which comprise opposing points of view since complicated concepts concerning the identity, religion, political or ideological leaning are the actual points where search engines are more likely to provide biased results~\citep{noble2018algorithms} and influence people dramatically.
%Because of the polarized viewpoints, controversial queries may contain sentiment-bearing keywords and punctuation or imply a specific sentiment pole. Hence, bias in the retrieved results could also be explained by the sentiment-bearing keywords present in the search query itself. 
%In order to make sure that our analysis is not affected by such sentiment-bearing queries, we measure bias using \emph{all} queries in the query set \(Q\), as well as using a restricted set of \emph{non-polarized} queries denoted by \(Q_{nonPol}\) as reported in the experimental results.

%pro means the news article's author, if asked about the topic, would answer  positively, e.g. being in favour of the topic.
%Neutral means that the news article author is only informative in nature and provides pro and cons of both perspectives, pro and against.
%Against means the news article's author, if asked about the topic, would answer negatively, e.g. being against of the topic.

Our second aim is to detect bias with respect to the distribution of ideological leanings expressed in the contents of the SERPs. We do this by associating each query $q \in \set{Q}$ belonging to a controversial topic to one \emph{current} ideological leaning. Then, combining the stances for each $r_i$ and the associated ideological leaning of $q$ we can measure the ideological bias of the content of a given SERP, e.g.~if a topic belongs to a specific ideology and a document retrieved for this topic has a pro stance, we consider this document to be biased towards this ideology.
We define the ideological leaning of $q$ as $j(q)$. An ideological leaning can have the following values:
\emph{conservative}, % (\bc), 
\emph{liberal}, % (\rc), 
\emph{both or neither}. % (\wc).

A topic ideological leaning can be:
\begin{itemize}
\item \textbf{conservative} ($\lcp\,$) when the topic is part of the conservative policies. The conservatives are in favour of the topic;
\item \textbf{liberal} ($\llp\,$) when the topic is part of the liberal policies. The liberals are in favour of the topic;
\item \textbf{both or neither} ($\lbp\,$) when both or neither policies are either in favour or against the topic.
\end{itemize}

\begin{table*}
\centering
\caption{Symbols, functions, and labels used throughout the paper}
\begin{tabular}{ l l }
\hline
\hline
{Symbols}\\
\hline
\hline
$\sS$   & set of search engines. \\
$s$     & a search engine $s \in \sS$. \\
$\sQ$   & set of queries. \\
$q$     & a query $q \in \sQ$. \\
%$d$     & a document. \\
$r$     & a ranked list of the given SERP (list of retrieved documents). \\%(list of documents).
$r_i$   & the document in $r$ retrieved at rank $i$.\\
$|r|$ & size of $r$ (number of documents in the ranked list). % = [r_1, r_2, \dots, r_{|r|}]$.
\\
$n$     & number of documents considered in $r$ %by $f$ 
(cut-off).\\
%$G$     & a set of groups $g_i$ ($g_1 \cup g_2 \cup \dots \cup g_n = G$). \\
%$g_i$   & a group $g_i \in G$. \\ \hline
%\hline
\hline
\hline
{Functions}\\
\hline
\hline
%$s(q)$                  & returns $r$ given a query ($q$). \\ 
$j(r_i)$                & returns the label associated to $r_i$.\\
%$j(q)$                  & returns the label associated to $q$.\\
$f(r)$                  & an evaluation measure for SERPs.\\
%$f_g(r)$                & like $f$ but for $g$.\\
%$f_{-}(r)$             & like $f$ but for the against label.\\
%$[\text{Condition}]$    & returns 1 if the condition is true and 0 otherwise.\\
\hline
\hline
{Labels}\\
\hline
\hline
%$g_1$  & protected group. \\
%$g_2$  & unprotected group. \\ \hline
$\lps$ & pro stance. \\
$\lns$ & neutral stance. \\
$\las$ & against stance. \\ 
$\lnr$ & not-relevant stance. \\ \hline
$\lcp$ & conservative ideological leaning.
\\
%$\lnp$ & neutral political perspective. \\
$\llp$ & liberal ideological leaning. \\
$\lbp$ & both or neither ideological leanings. \\
%$+$ & label  .\\
%$-$ & against label.\\
\hline
\hline
\end{tabular}
\label{table:notation}
\end{table*}

For reference, Table~\ref{table:notation} shows a summary of all the symbols, functions and labels used in this paper. 
%\subsection{Extracting Stances}

% EMINE: Is it possible to report some numbers for the accuracy of TextBlob?
%To extract the perspective of a given opinionated text we use crowdsourcing. {\color{red} TODO}.
%To extract the sentiment orientation of a given opinionated text, we use the TextBlob API~\cite{TextBlob2017} which is a publicly available, stable and handy python library that stands on NLTK~\cite{bird2009natural} and pattern\footnote{https://www.clips.uantwerpen.be/pattern} modules for various natural language processing tasks such as part-of-speech tagging, noun phrase extraction, and sentiment analysis. TextBlob  uses a Naive Bayes predictor on an annotated dataset and it is a reliable resource for sentiment analysis. We extract sentiment information of a given text via TextBlob at document and sentence levels.

%\textbf{Document-level:} 
%For each query $q \in \set{Q}$ of the search engine $s$, we first obtain a perspective value $j(d, q)$ for each $d \in \set{D}$ %from TextBlob without any preprocessing step on documents since TextBlob handles the punctuation, tokenisation, etc.  As the output, we have a set of  sentiment values of all \(d_{i_{k}} \in D_i\) retrieved by \(S_j\), denoted as \(Pol_{S_j} ({q_i}) =  \{s(d_{i_{1}}), s(d_{i_{2}}), ...., s(d_{i_{n}})\}\). The \emph{document-level} sentiment analysis is more coarse-grained compared to \emph{sentence-level} which will be explained in the following section. 

%\textbf{Sentence-level:} Each document is viewed as a pile of sentences. We first split each document \(d\) into its \emph{m} sentences and denote the set of sentences for the document \(d\) as \(STC(d) = \{s_{1}, s_{2}, .... , s_{m}\}\). For each sentence \(s_{l} \in 
%STC(d)\), we obtain a polarity value \(s(s_{l})\) from TextBlob. The set of sentiment values of all \emph{sentences} in the given document \(d\) is denoted by \(SentPol_d = \{s(s_{1}), s(s_{2}), .... , s(s_{m})\}\). We then compute an average over all the sentence polarity values in \(SentPol_{d}\) and generate the document polarity score of the document \(d\) as \(s_{pol}(d)\). In the same way, we calculate the polarities of all documents \(d_{i_{k}} \in D_i\) and denote the set of sentence-level document polarities as \(SentPol_{S_j} (q_i) = \{s_{pol}(d_{i_{1}}), s_{pol}(d_{i_{2}}), ...., s_{pol}(d_{i_{m}})\}\). Sentence-level analysis enables us to concentrate on the opinions expressed in the sentences rather than only seeing a document as a whole.
%Owing to this more fine-grained analysis comparing to the \textit{document-level}, we aim to incorporate the sentence-level sentiments of the opinions expressed in the SERPs into our framework.

%%\subsection{Sentiment to Perspective Transformation and Normalization}\label{transformation}

%%After calculating the sentiment polarity of a document, we need a way to exploit that information in measuring bias. Since we are dealing with controversial queries with different conservative and liberal perspectives, we transform the polarity values from \emph{negative-positive} scale to \emph{conservative-liberal} scale for consistency. This transformation is needed because there may be documents which express positive sentiment, lets say, towards \emph{abortion} and \emph{Cuba embargo}. Though these documents have the same sentiment polarity, they have different leanings since having \emph{positive} opinion on \emph{abortion} implies a \textit{liberal-leaning}, whereas a positive opinion on \emph{Cuba embargo} implies a \emph{conservative-leaning}. For some queries (as in the case of \emph{abortion}), we can directly interpret the \emph{negative-positive} sentiment polarity values of SERPs as \emph{conservative-liberal} leaning scores while for other queries (as in the case of the \emph{Cuba embargo}), we need to revert the sentiment polarity values of SERPs by multiplying them by -1 to obtain \emph{conservative-liberal} leaning scores. On the other hand, for some queries such as \emph{Vegetarianism} conservative-liberal perspectives are not apparent and therefore \emph{negative-positive} sentiment polarity values are interpreted as general negative and positive leaning  without reverting. We denote this simple mapping of SERP sentiment polarities to leaning scores as \(TRSFM\). Queries which need their SERP sentiment polarity values to be multiplied by -1 are decided by three human annotators with majority-voting since this task requires human expertise. 
%if the leaning (conservative, or %liberal) of a document in the %query's list can be determined  by %the annotator and the document %conveys a highly positive or %negative sentiment towards that %query. Queries to be transformed are %selected by three human annotators %with majority-voting.
%For some of the bias measures, we need to normalize the leaning scores. For those scores we use well-known min-max normalization to map them to [0, 1] range. We denote this normalization function by \(NRMZ\). Sentiment-based metrics which require normalized \emph{conservative-liberal} leaning scores are explained in Section~\ref{SentimentMetrics}, and quantification of bias using these metrics is explained in Section~\ref{BiasQuantification}.

\subsection{Measures of Bias}
\label{sec:measuresbias}

Based on the aforementioned definition provided in Section \ref{sec:introduction}, bias can be quantified by measuring the degree of deviation of the distribution of documents from the \textit{ideal} one. To give a broad definition of an ideal list poses problems; but in the scope of this work for \emph{controversial} topics, we can mention the existence of bias in a ranked list retrieved by a search engine if the presented information \emph{significantly deviates} from true likelihoods~\citep{white2013beliefs}. 
As justified in Section~\ref{sec:introduction}, in the scope of this work we focus on~\emph{equality of output}, thus we accept the true likelihoods of different views as \emph{equal} rather than computing them from the corresponding base rates.
Therefore using the proposed definition reversely, we can assume that the \textit{ideal} list is the one that minimises the difference between two opposing views, which we indicate here as $\lps$ and $\las$ in the context of stances.
%form the \emph{unbiased} lists by \emph{randomly} generating the ranked document lists and accept them as \textit{IDEAL} lists for our framework. 
%Then for quantifying bias, we measure the difference between the ranked lists returned from the two search engines 
%, Bing and Google and the \textit{IDEAL} list in terms of the proposed sentiment-based metrics. The steps of the overall procedure for quantifying bias in SERPs is as follows. 
%
%Our aim is to detect the existence of bias in SERPs of a search engine as well as to compare the SERPs of two search engines in terms of bias with respect to controversial topics.
Formally, we measure the \emph{stance} bias in a SERP $r$ as follows:
%
\begin{linenomath*}
\begin{equation}\label{eq:bias}
    \beta_f(r) = f_{\lps}(r) - f_{\las}(r),
\end{equation}
\end{linenomath*}
%
where $f$ is a function that measures the likelihood of $r$ in satisfying the information need of the user about the view $\lps$ and the view $\las$. We note that \emph{ideological} bias is measured in the same way by transforming the stances of the documents into ideological leanings which will be explained in Section \ref{sec:crowdsourcing}.
Before defining $f$, from Eq.~\eqref{eq:bias}, we define the mean bias (MB) of a search engine $s$ as:
%
\begin{linenomath*}
\begin{equation*}\label{eq:expected_biasMB}
    \text{MB}_f(s, \sQ) = 
    \frac{1}{|\sQ|}
    \sum_{q \in \sQ} \beta_f(s(q)).
\end{equation*}
\end{linenomath*}
%
An unbiased search engine would produce a mean bias of $0$. 
A limitation of MB is that if a search engine is biased towards the $\lps$ view on one topic and bias towards the $\las$ view on another topic, these two contributions will cancel each other out. 
In order to avoid this limitation we also define the mean absolute bias (MAB), which consists in taking the absolute value of the bias for each $r$. Formally, this is defined as follows:
%
\begin{linenomath*}
\begin{equation}\label{eq:expected_biasMAB}
    \text{MAB}_f(s, \sQ) = 
    \frac{1}{|\sQ|}
    \sum_{q \in \sQ} |\beta_f(s(q))|.
\end{equation}
\end{linenomath*}
%
An unbiased search engine produces a mean absolute bias of $0$. Although this measure defined in Eq.~\eqref{eq:expected_biasMAB} solves the limitation of MB, MAB says nothing about towards which view the search engine is biased, making these two measures of bias complementary.

In IR the likelihood of $r$ in satisfying the information need of users is measured via retrieval evaluation measures. Among these measures we selected 3 \emph{utility-based} evaluation measures. This class of evaluation measures quantify $r$ in terms of its worth to the user and are normally computed as a sum of the information gain summed over the relevant documents retrieved by $r$. 
The 3 IR evaluation measures used in the following experiments are: 
P$@n$, RBP, and DCG$@n$.

P$@n$ for the $\lps$ view is formalised as in Eq. \eqref{eq:pc}. %the ratio between the relevant retrieved documents over the cut-off $n$. To quantify the bias towards one view we reformulate P$@n$ as the ratio between the relevant retrieved documents for the view over the cut-off $n$. For example, for the $+$ view, this is formalized as follows:
%
%\begin{equation}\label{eq:pc}
%    \text{P}_+@n = 
%    \frac{1}{n}\sum_{i=1}^n 
%    [j(r_i) = +]
%\end{equation}
%
%where the notation $[Condition]$ (aka Iverson bracket) returns 1 when the condition is verified and 0 when otherwise. $j(r_i)$ returns the stance of the document with respect to the topic $q$. 
However, differently from the previous definition of $j(r_i)$ where the only possible outcomes are $g_1$ and $g_2$ for the document $r_i$, here $j$ can return any of the label associated to a stance ($\lps$, $\lns$, $\las$, and $\lnr$). Hence, only pro and against documents, that are relevant to the topic, are taken into account, since $j(r_i)$ returns \emph{neutral} and \emph{not-relevant} when otherwise.
Substituting Eq.~\eqref{eq:pc} to Eq.~\eqref{eq:bias} we obtain the first measure of bias:
%
\begin{linenomath*}
\begin{equation*}\label{eq:bias_pc}
    \beta_{\text{P}@n}(r) = 
    \frac{1}{n}\sum_{i=1}^n 
    \left([j(r_i) = \lps] - [j(r_i) = \las]\right).
\end{equation*}
\end{linenomath*}
%
The main limitation of this measure of bias is that it has a weak concept of ranking, 
i.e.~the first $n$ documents contribute equally to the bias score. The next two evaluation measures overcome this issue by defining discount functions.

RBP weights every document based on the coefficients of a normalised geometric series with value $p \in ]0,1[$, where $p$ is a parameter of RBP. Similarly to what is done for P$@n$, we reformulate RBP to measure bias as follows:
%
\begin{linenomath*}
\begin{equation}\label{eq:rbpc}
    \text{RBP}_{\lps} = 
    (1-p) 
    \sum_{i=1} p^{i-1}[j(r_i) = \lps].
\end{equation}
\end{linenomath*}
%
Substituting Eq.~\eqref{eq:rbpc} to Eq.~\eqref{eq:bias} we obtain:
%
\begin{linenomath*}
\begin{equation*}\label{eq:bias_rbpc}
    \beta_{\text{RBP}}(r) = (1-p) \sum_{i=1} p^{i-1} \left(
    [j(r_i) = \lps] - [j(r_i) = \las]
    \right).
\end{equation*}
\end{linenomath*}
%
DCG$@n$, instead, weights each document based on a logarithmic discount function. Similarly to what is done for P$@n$ and RBP, we reformulate DCG$@n$ to measure bias as follows:
%
\begin{linenomath*}
\begin{equation}\label{eq:dcgc}
    \text{DCG}_{\lps}@n = \sum_{i=1}^{n} 
    \frac{1}{\log(i + 1)}[j(r_i) = \lps].
\end{equation}
\end{linenomath*}
%
Substituting Eq.~\eqref{eq:dcgc} to Eq.~\eqref{eq:bias} we obtain:
%
\begin{linenomath*}
\begin{equation}\label{eq:bias_dcg}
    \beta_{\text{DCG}@n}(r) = \sum_{i=1}^{n}
    \frac{1}{\log(i + 1)}\left(
    [j(r_i) = \lps] - [j(r_i) = \las]
    \right)
\end{equation}
\end{linenomath*}
%

Since we are evaluating web-users, for P$@n$ and DCG$@n$ we set $n=10$ and for RBP we set $p = 0.8$. This last formulation (Eq.~\eqref{eq:bias_dcg}), although it looks similar to the rND measure, it does not suffer from the four limitations introduced in Section \ref{subsec:fairness_evaluation}. 
In particular all these presented measures of bias:
1) do not focus on one group;
2) use a binary score associated to the document stance or ideological leaning, similar to the way these measures are used in IR when considering relevance; also like in IR  
3) can be computed at each rank; 
4) exclude non-relevant documents from the measurement of bias and; the framework
5) provides various user models associated to the 3 IR evaluation measures: P$@n$, DCG$@n$, and RBP.
%\end{enumerate}
%\subsection{Sentiment-Based Metrics}
%\label{SentimentMetrics}

%\(\mathbf{AVG_{Senti}}\) is based on the document and sentence-level average sentiment scores. For the document-level score of a search engine \(S_j\) for query \(q_i\), we calculate the mean over all the document sentiment polarities \(s(d_{i_{k}}) \in Pol_{S_j} (q_i)\) for the documents \(d_{i_{k}} \in D_i\) retrieved by \(S_j\) and denote it as \(AvgPol_{doc} (q_i, S_j)\). To calculate a sentence-level score, we find an average over all the sentence-level document polarities \(s_{pol}(d_{i_{k}}) \in SentPol_{S_j}({q_i})\) for all the documents and denote it by \(AvgPol_{sent} (q_i,S_j)\). This metric only measures the sentiment distribution in the given ranked list without considering rank information.

%{\color{red}
%\(\mathbf{NDCG_{Senti}}\) integrates the sentiment distribution and rank of the documents in a given ranked list which is a variant of the commonly used NDCG metric displayed in Eq.~\ref{eq:dcg_ndcg} where \(p\) stands for the \emph{rank} (of a document) and \(rel_i\) is the \emph{relevance} score of the document at rank \(i\). The \(DCG\) and the Ideal \(DCG\) (\(IDCG\)) are computed on the same list where \(IDCG\) computes the \(DCG\) of the best possible ranking of the same list  (i.e. most relevant documents are at higher rankings).
%\vspace{-0.2cm}
%\begin{equation}
%NDCG_p = \frac{DCG_p}{IDCG_p}, DCG_p = rel_1 + \sum_{i=2}^{p} \frac{rel_i}{\lo\las(i)}
%\label{eq:dcg_ndcg}
%\vspace{-0.1cm}
%\end{equation}}

%\(\mathbf{DCG_{Senti}}\) integrates the sentiment distribution and rank of the documents in a given ranked list which is a variant of the commonly used NDCG metric displayed in Eq.~\ref{eq:dcg_ndcg} where \(p\) stands for the \emph{rank} (of a document) and \(rel_i\) is the \emph{relevance} score of the document at rank \(i\).
%\vspace{-0.2cm}
%\begin{equation}
%DCG_p = rel_1 + \sum_{i=2}^{p} \frac{rel_i}{\lo\las(i)}
%\label{eq:dcg_ndcg}
%\vspace{-0.1cm}
%\end{equation}

%Add P@10

%RBP rank biased precision 
%\begin{equation}
%    RBP = (1-p)\sum_{i = 1} p^{i-1} rel_i
%\end{equation}

%Before computing the \(NDCG_{Senti}\), since the relevance grades are always positive, we need to apply the \(NRMZ\) on the transformed sentiment polarities. After having applied the \(NRMZ\), we obtain normalized sentiment polarities in the range of \([0,1]\). Then, we interpret the normalized polarity scores as the probabilities of relevance and replace the relevance scores \(rel_i\) in the formula with these normalized sentiment values. To compute the document and sentence-level \(NDCG_{Senti}\) metric scores, we use the document polarities in the same way as we did in the \(AVG_{Senti}\). We denote the document and sentence-level \(NDCG_{Senti}\) scores respectively as \(NDCG_{doc} (q_i, S_j)\) and \(NDCG_{stc} (q_i, S_j) \) for the given query \(q_i\) and search engine \(S_j\).

%{\color{red}
%\(\mathbf{AP_{Senti}}\) computes an average precision score for a given ranked list of documents. Since the polarity scores can be in the range of 0 to 1, we use an alternative version of the metric that can accept probabilistic relevance scores, as proposed in~\cite{aslam2005maximum} as shown in Eq.2.
%\vspace{-0.2cm}
%\begin{equation}
%AP_p = \frac{1}{R} \, \sum_{i=1}^{p} \, ( \, \frac{p_i}{i} (1 \, + \, \sum_{j=1}^{i-1}p_j \, ))
%\label{eq:ap}
%\vspace{-0.2cm}
%\end{equation}
%}

%Similarly to \(NDCG_{Senti}\), before the computation of \(AP_{Senti}\), we normalize the already transformed sentiment polarities and map them onto \([0,1]\). Then, we interpret the \(normalized\) sentiment polarities as probabilities and use these \(normalized\) values instead of \(p_i\) and \(p_j\) probability scores in the formula to calculate \(AP_{Senti}\). The document and sentence-level \(AP_{Senti}\) scores are denoted respectively as \(AP_{doc} (q_i, S_j)\) and \(AP_{sent} (q_i, S_j)\) for the given query \(q_i\) and search engine \(S_j\). As seen from the formula, this metric also combines sentiment and position information, but differently from \(NDCG_{Senti}\).

\subsection{Quantifying Bias}
\label{sec:protocol}
Using the measures of bias defined in the previous section we quantify the bias of the two search engines, Bing and Google using the \emph{news versions} of these search engines. % against an \textit{ideal} stance distribution.
Then, we compare them thereof. Following, we describe each step of the proposed procedure used to quantify bias in SERPs.
%
\begin{itemize}
\item \textbf{News Articles in SERPs.}
We obtained the controversial queries
issued for searching from ProCong.org [2018] and applied
some filtering steps on the initial query set. After filtering,
the final query set size became 57. We submitted each query
in the final query set to the US News search engines of
Google and Bing using a US proxy. Then, we extracted the
whole corpus returned by both engines in response to all
the queries in the set. Note that the data collection process
was done in a controlled environment such that the queries
are sent to the search engines at the same time. For more
details about the selection of the queries and crawling the
SERPs, please refer to the previous phase of our analysis.
After having crawled all the SERPs returned from both engines and extracted their contents, we annotated the top 10
documents. We obtained the stance label of each document
with respect to the queries via crowd-sourcing. To label the
ideological leaning of queries, we also used crowd-sourcing.
To obtain the ideologies of documents, we transformed the
stance labels into ideologies based on the ideological leaning
of their corresponding queries. The details about our crowdsourcing campaigns as well as the transformation process
can also be found in the first phase of our analysis.

%
\item \textbf{Bias Evaluation.}
We compute the bias measures for every SERP with all three IR-based measures of bias: P$@n$, RBP, and DCG$@n$. 
We then aggregate the results using the two measures of bias, MB and MAB. % polarity scores from TextBlob in document and sentence-level as \(Pol_{S_j} ({q_i})\), and \(SentPol_{S_j}({q_i})\) respectively for all the queries \(q_i\). Then, we apply \(TRSFM\) function on these scores.
%After the transformation, we directly compute \(AvgPol_{doc} (q_i, S_j)\) and \(AvgPol_{sent} (q_i, S_j)\) scores. Further, we also apply \(NRMZ\) on the transformed sentiment values. After that we compute \(NDCG_{doc} (q_i, S_j)\), \(AP_{doc} (q_i, S_j)\), \(NDCG_{stc} (q_i, S_j)\) and \(AP_{sent} (q_i, S_j)\) scores since negative values cause problems in the computation. Now, to quantify bias, we need to generate an ideal list and measure the deviation of the SERPs of two search engines. For distinguishing the differences in their viewpoints, we only compare the computed metric scores.
%
%\item \textbf{\textit{Ideal} List Generation:}
%To constitute an ideal list, we randomly generate 50 ranked lists where each list is composed of 10 documents. Since in our framework documents are associated with sentiment polarity scores which are used for measuring bias, we randomly generate only polarity values. After applyin the NRMZ function, all the sentiment scores obtained from TextBlob are mapped to [0, 1] range, therefore the sentiment scores are also randomly chosen from \{0, 1\} for consistency.
%
%\item \textbf{\textit{Ideal} Computation of the Sentiment-Based Metrics:}
%For our first metric, \(AVG_{Senti}\), we do not need to generate an \textit{IDEAL} list since in the scope of \(AVG_{Senti}\), it is straightforward. We do not apply \(NRMZ\) but only \(TRSFM\) on the sentiment values to compute \(AVG_{Senti}\), therefore we have both positive and negative values in our list for any query \(q_i\). Hence, the \textit{IDEAL} list should have a balanced distribution of positive and negative documents meaning that the document and sentence-level \(AVG_{Senti}\) score of the ideal list should be 0. On the other hand, differently from \(AVG_{Senti}\), we both apply \(TRSFM\) and \(NRMZ\) to calculate \(NDCG_{Senti}\) and \(AP_{Senti}\) scores and it is more difficult to define an ideal list for them. Therefore, we form the \textit{IDEAL} list by utilizing ``randomized ranking''. We compute the \(NDCG_{Senti}\) and \(AP_{Senti}\) for each of the 50 randomly generated lists and calculate two average scores, namely ideal \(NDCG_{Senti}\) and \(AP_{Senti}\) in our framework.
%\textcolor{red}{Check here}
\item \textbf{Statistical Analysis.}
To identify whether the bias measured is not a byproduct of randomness, 
%for the bias measure MAB, 
we compute a one-sample t-test: 
the null hypothesis is that no difference exists and that the true mean is equal to zero. 
%
If this hypothesis is rejected, hence there is a significant difference and we claim that the evaluated search engine is biased.
%
%Then, to find out towards which view the search engine is biased and show this is not due to noise, we compute a one-sample t-test on the bias measure MB: the null hypothesis is that no difference exists (between two opposing views) and that the true mean is equal to zero.
%
%Additionally, we compare the difference in bias measured across the two search engines, for both of the measures of MB and MAB, using a two-tailed paired t-test: the null hypothesis is that the difference between the two true means is equal to zero.
%
%If this hypothesis is rejected, hence there is a significant difference and we claim that there is a difference in bias between the two search engines.
%
Then, we compare the difference in bias measured across the two search engines using a two-tailed paired t-test: the null hypothesis is that the difference between the two true means is equal to zero. If this hypothesis is rejected, hence there is a significant difference, we claim that there is a difference in bias between the two search engines.
\end{itemize}

\
